On the Distribution of Partially Symmetric Codes for Automorphism Ensemble Decoding

Automorphism Ensemble (AE) decoding has recently drawn attention as a possible alternative to list decoding of polar codes. In this letter, we investigate the distribution of Partially-Symmetric Reed-Muller (PS-RM) codes, a family of polar codes yielding good performances under AE decoding. We prove the existence of these codes for almost all code dimensions for code lengths $N\leq 256$. Moreover, we analyze the absorption group of this family of codes under SC decoding, proving that valuable permutations in AE decoding always exist. Finally, we experimentally show that PS-RM codes can outperform state-of-the-art polar-code-construction algorithms in terms of error-correction performance for short code lengths, while reducing decoding latency.

==> figures/percentage.tex <==
\begin{tikzpicture}
%   \pgfplotsset{
%     label style = {font=\fontsize{9pt}{7.2}\selectfont},
%     tick label style = {font=\fontsize{9pt}{7.2}\selectfont}
%   }

  \begin{axis}[%
    width=\columnwidth,
    height=0.450\columnwidth,
    xmin=1, xmax=8,
    xtick={1,2,...,8},
    %xticklabels={{$2$},{$2.5$},{$3$},{$3.5$},{$4$}},
    xlabel={Symmetry $t$},
    xlabel style={yshift=0.4em},
    ymin=0, ymax=40,
    ylabel style={yshift=-3mm},
    ylabel={Percentage},
    yminorticks, xmajorgrids,
    ymajorgrids, yminorgrids,
    %position
    legend style={at={(1,1)},anchor=north east},
    %column font, row sep
    legend style={legend columns=1, font=\small, row sep=-1.2mm},
    legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1}, % for future use maybe ? %opacity of filling/border and inside text
    legend style={inner xsep=0.5pt, inner ysep=0.5pt}, % TIGHTER BORDER !!!!!
    legend cell align={right}, % avoid centering in legend
    mark size=1.6pt, mark options=solid,
    ]

        
    

    \addplot[color=matlab1, mark=10-pointed star, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    19.05\\
    2.0000    38.10\\
    3.0000    19.05\\
    4.0000    9.52\\
    5.0000    14.29\\
    6.0000         0\\
   % 7.0000         0\\
    %8.0000         0\\
    };
    \addlegendentry{$N=32$}
    \addplot[color=matlab2, mark=x, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    7.84\\
    2.0000    35.29\\
    3.0000    31.37\\
    4.0000    11.76\\
    5.0000    5.88\\
    6.0000    7.84\\
    7.0000         0\\
    %8.0000         0\\
};
    \addlegendentry{$N=64$}
    \addplot[color=matlab3, mark=diamond, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    4.42\\
    2.0000    23.89\\
    3.0000    34.51\\
    4.0000    21.24\\
    5.0000    7.96\\
    6.0000    3.54\\
    7.0000    4.42\\
    8.0000         0\\
    };
    \addlegendentry{$N=128$}
    
     \addplot[color=matlab4, mark=o, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    2.93\\
    2.0000    17.57\\
    3.0000    27.20\\
    4.0000    30.96\\
    5.0000    12.13\\
    6.0000    4.60\\
    7.0000    2.09\\
    8.0000    2.51\\
};
    \addlegendentry{$N=256$}
  \end{axis}

\end{tikzpicture}%


    

==> figures/percentage_bar.tex <==
\begin{tikzpicture}
%   \pgfplotsset{
%     label style = {font=\fontsize{9pt}{7.2}\selectfont},
%     tick label style = {font=\fontsize{9pt}{7.2}\selectfont}
%   }

  \begin{axis}[
    ybar,
    width=\columnwidth,
    height=0.450\columnwidth,
    xmin=1, xmax=8,
    xminortick={1,2,...,8},
    %xticklabels={{$2$},{$2.5$},{$3$},{$3.5$},{$4$}},
    xlabel={Symmetry $t$},
    xlabel style={yshift=0.4em},
    ymin=0, ymax=40,
    ylabel style={yshift=-3mm},
    ylabel={Percentage},
    xminorticks, xminorgrids
    ymajorgrids%, yminorgrids,
    %position
    legend style={at={(1,1)},anchor=north east},
    %column font, row sep
    legend style={legend columns=1, font=\small, row sep=-1.2mm},
    legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1}, % for future use maybe ? %opacity of filling/border and inside text
    legend style={inner xsep=0.5pt, inner ysep=0.5pt}, % TIGHTER BORDER !!!!!
    legend cell align={right}, % avoid centering in legend
    mark size=1.6pt, mark options=solid,
    ]

        
    

    \addplot[color=matlab1, line width=0.8pt, draw=black,fill=matlab1]
    coordinates{
    1.0000    19.05\\
    2.0000    38.10\\
    3.0000    19.05\\
    4.0000    9.52\\
    5.0000    14.29\\
    6.0000         0\\
   % 7.0000         0\\
    %8.0000         0\\
    };
    \addlegendentry{$N=32$}
    \addplot[color=matlab2, mark=x, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    7.84\\
    2.0000    35.29\\
    3.0000    31.37\\
    4.0000    11.76\\
    5.0000    5.88\\
    6.0000    7.84\\
    7.0000         0\\
    %8.0000         0\\
};
    \addlegendentry{$N=64$}
    \addplot[color=matlab3, mark=diamond, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    4.42\\
    2.0000    23.89\\
    3.0000    34.51\\
    4.0000    21.24\\
    5.0000    7.96\\
    6.0000    3.54\\
    7.0000    4.42\\
    8.0000         0\\
    };
    \addlegendentry{$N=128$}
    
     \addplot[color=matlab4, mark=o, line width=0.8pt, mark size=2.8pt]
    table[row sep=crcr]{%
    1.0000    2.93\\
    2.0000    17.57\\
    3.0000    27.20\\
    4.0000    30.96\\
    5.0000    12.13\\
    6.0000    4.60\\
    7.0000    2.09\\
    8.0000    2.51\\
};
    \addlegendentry{$N=256$}
  \end{axis}

\end{tikzpicture}%


    
